SkySenseGPT: A Fine-Grained Instruction Tuning Dataset and Model for Remote Sensing Vision-Language Understanding

Remote Sensing Large Multi-Modal Models (RSLMMs) are developing rapidly and showcase significant capabilities in remote sensing imagery (RSI) comprehension. However, due to the limitations of existing datasets, RSLMMs have shortcomings in understanding the rich semantic relations among objects in complex remote sensing scenes. To unlock RSLMMs' complex comprehension ability, we propose a large-scale instruction tuning dataset FIT-RS, containing 1,800,851 instruction samples. FIT-RS covers common interpretation tasks and innovatively introduces several complex comprehension tasks of escalating difficulty, ranging from relation reasoning to image-level scene graph generation. Based on FIT-RS, we build the FIT-RSFG benchmark. Furthermore, we establish a new benchmark to evaluate the fine-grained relation comprehension capabilities of LMMs, named FIT-RSRC. Based on combined instruction data, we propose SkySenseGPT, which achieves outstanding performance on both public datasets and FIT-RSFG, surpassing existing RSLMMs. We hope the FIT-RS dataset can enhance the relation comprehension capability of RSLMMs and provide a large-scale fine-grained data source for the remote sensing community. The dataset will be available at https://github.com/Luo-Z13/SkySenseGPT

==> tables/region_caption_instruction.tex <==
\begin{table*}[h!]
% \footnotesize
\centering

\label{tab:region_caption_instruction_old}
    
\begin{minipage}{\linewidth}
\begin{tcolorbox} 
\begin{tabular}{p{\linewidth}}
\begin{itemize}[left=0pt]
\vspace{-0.5em}
    \item "Can you provide me with a detailed description of the region in the image marked by <region>?"
    \item "I'm curious about the region represented by <region> in the picture. Could you describe it in detail?"
    \item "What can you tell me about the region indicated by <region> in the image?"
    \item "I'd like to know more about the area in the photo labeled <region>. Can you give me a detailed description?"
    \item "Could you describe the region shown as <region> in the picture in great detail?"
    \item "What details can you give me about the region outlined by <region> in the photo?"
    \item "Please provide me with a comprehensive description of the region marked with <region> in the image."
    \item "Can you give me a detailed account of the region labeled as <region> in the picture?"
    \item "I'm interested in learning more about the region represented by <region> in the photo. Can you describe it in detail?"
    \item "What is the region outlined by <region> in the picture like? Could you give me a detailed description?"
    \item "Can you provide me with a detailed description of the region in the picture marked by <region>, please?"
    \item "Please provide a detailed description of the region <region> in the given image."
    \item "What can you tell me about the region indicated by <region> in the image, exactly?"
    \item "I'd like to know more about the area in the photo labeled <region>, please. Can you give me a detailed description?"
    \item "Could you describe the region shown as <region> in the picture in great detail, please?"
    \item "Please provide me with a comprehensive description of the region marked with <region> in the image, please."
    \item "Can you give me a detailed account of the region labeled as <region> in the picture, please?"
    \item "I'm interested in learning more about the region represented by <region> in the photo. Can you describe it in detail, please?"
    \item "What is the region outlined by <region> in the picture like, please? Could you give me a detailed description?"
    \item "Please describe the region <region> in the image in detail."
    \item "Can you offer a thorough analysis of the region <region> in the image?"
    \item "Could you elaborate on the region highlighted by <region> in the picture provided?"
    \item "Please share more information about the zone emphasized with <region> in the photo."
    \item "What insights can you give about the area denoted by <region> in the image presented?"
    \item "Can you share a comprehensive rundown of the region denoted by <region> in the presented image?"
    \item "I'd like to know more about the region highlighted by <region> in the picture provided."
    \item "Work through the important details of the area <region> in the image."
    \item "Illustrate the area represented by <region> through a descriptive explanation."
    \item "Examine the region <region> closely and share its details."
\end{itemize}

\end{tabular}
\end{tcolorbox}
\end{minipage}
\caption{The list of instructions for detailed region caption.
}
\end{table*}

